Open Problems and Modern Solutions for Deep Reinforcement Learning

Deep Reinforcement Learning (DRL) has achieved great success in solving complicated decision-making problems. Despite the successes, DRL is frequently criticized for many reasons, e.g., data inefficient, inflexible and intractable reward design. In this paper, we review two publications that investigate the mentioned issues of DRL and propose effective solutions. One designs the reward for human-robot collaboration by combining the manually designed extrinsic reward with a parameterized intrinsic reward function via the deterministic policy gradient, which improves the task performance and guarantees a stronger obstacle avoidance. The other one applies selective attention and particle filters to rapidly and flexibly attend to and select crucial pre-learned features for DRL using approximate inference instead of backpropagation, thereby improving the efficiency and flexibility of DRL. Potential avenues for future work in both domains are discussed in this paper.

==> numericalresults.tex <==
\section{Numerical Experiments}
\label{Numerical_Experiments}
%
To compare the optimal values of problem~\eqref{eqn_problem1} and problem~\eqref{eqn_problem2_mirror}, we consider a continuous navigation task in an environment populated with hazardous obstacles (see Figure~\ref{configuration}). The coordinates of the obstacles' centers are (7, 7), (3, 7), (1.5, 4), (4.5, 3), (8, 3) with the corresponding radii \{2, 1, 0.5, 1.5, 0.75\}. The state in this example  is  the position of the agent on the $x-$ and $y-$axis, namely, $s=(x, y)$. We set the continuous state space as $\mathcal{S}=[0, 10] \times [0, 10]$. The goal of the agent is to reach a goal position $s_{goal}=(9, 1.5)$ within the time horizon $T=20$, while avoiding 5 obstacles. Accordingly, the safe set is defined as the whole map/state space excluding regions of 5 obstacles.

The agent's action $a$ is a two-dimensional velocity. For a given state and action at time $t$, the state evolves according to $s_{t+1}=s_t+ a_t T_s$ with $T_s=0.05$. The policy of the agent is a multivariate Gaussian distribution
%
\begin{align}\label{gaussian_policy}
    \pi_\theta (a | s)\! =\! \frac{1}{\sqrt{2\pi |\Sigma|}} \exp \! \left(\! -\frac{1}{2} \left(a-\mu_\theta(s)\right)^\top \!\! \Sigma^{-1} \!\! \left(a-\mu_\theta(s)\right) \! \right),
\end{align}
where $\mu_\theta(s)$ and $\Sigma$ denote the mean and covariance matrix of the Gaussian policy. We parameterize $\mu_{\theta}(s)$ as a linear combination of Radial Basis Functions (RBFs) 
\begin{align}\label{RBF}
    \mu_\theta (s) = \sum_{k=1}^{d} \theta_k \exp \left(-\frac{||s-\Bar{s}_k||^2}{2\sigma^2} \right),
\end{align}
where $\theta = [\theta_1, \theta_2, \cdots, \theta_d]^\top$ are parameters that need to be learned, $\Bar{s}_k$ are centers of each RBFs kernel and $\sigma$ their bandwidth. In this experiment we set $\Sigma = \text{diag} (0.5, 0.5)$, $\sigma =0.5$, $d=1681$  and $\Bar{s}_k = (x_k, y_k),  k=1, 2, \cdots, 1681$ where $\Bar{s}_k$ forms a uniform lattice with separation $0.25$ in each direction.
%

The reward is the negative squared distance to the goal position $s_{goal}$, i.e., $r(s_t, a_t)= -\lVert s_t - s_{goal} \rVert^2$. 
%%
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/configuration.png}
\caption{Navigation policy learned after 40,000 iterations for probabilistic constraint formulation selecting $\lambda=6, \eta = 0.002$. The agent is trained to navigate starting from (1, 8.5) to a goal (9, 1.5).}
\label{configuration}
\end{figure} 
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/safety_return.png}
\caption{Depicted in blue is the safety-reward for the cumulative constraint formulation \eqref{eqn_relaxation_2} for different values of $\mu\in[0.45,14]$ applied to the navigation problem depicted in Figure \ref{configuration}. Depicted in red is the safety-reward for the probabilistic constraint formulation \eqref{eqn_agmt_obj} for different values of $\lambda\in[0.45,14]$ applied to the navigation problem depicted in Figure \ref{configuration}. As it can be observed the probabilistic constraint traces a better trade-off of reward and safety as defined in Definition \ref{definition_safety}.}
\label{safety_vs_reward}
\end{figure}
%
%
We attempt to find solutions to \eqref{eqn_problem1} and \eqref{eqn_problem2_mirror} through regularization. This is, instead of solving \eqref{eqn_problem1} we consider the regularized version in \eqref{eqn_agmt_obj} and instead of \eqref{eqn_problem2_mirror} the following regularization of the constraints
%
\begin{equation}\label{eqn_relaxation_2}
    V_\mu(\theta) = \mathbb{E} \left[\sum\limits_{t=0}^{T} \Big(r(S_t,A_t) + \mu \mathds{1} ( S_t \in \mathcal{S}_\text{safe}) \Big) |\pi_\theta \right],
\end{equation}
%
where $\mu$ is a parameter that trades-off the reward for safety. For large $\mu$ policies are induced to be excessively safe, whereas if $\mu$ is small the agent is more concerned with rewards.

As claimed by Theorem~\ref{corollary_P_star_Ptilder_star} for the same level of safety the probabilistic formulation \eqref{eqn_problem1} yields a value that is always larger than the CMDP formulation \eqref{eqn_problem2_mirror}. Therefore we expect both formulations to trace different Pareto fronts as we modify the hyper-parameters $\lambda$ and $\mu$ in \eqref{eqn_agmt_obj} and \eqref{eqn_relaxation_2}. 

To solve \eqref{eqn_relaxation_2} we define the reward 
\begin{equation}\label{eqn_reward_risk}
   r_\mu(S_t, A_t)=r(S_t, A_t) + \mu \mathds{1} ( S_t \in \mathcal{S}_\text{safe}),
\end{equation}
and we consider off-the-shelf reinforcement learning algorithms. In particular, we consider a stochastic approximation of the Policy Gradient Theorem which yields the following update rule for the parameters $\theta$ of the policy
\begin{align}\label{update_rule_cumulative}
    \theta_{k+1} &=\theta_k + \eta  \hat{\nabla} V_\mu (\theta) \nonumber \\
    &= \theta_k+\eta\left(\sum\limits_{t=0}^{T-1} R_{t,\mu} \nabla_{\theta}\log\pi_\theta(A_t\mid S_t) \right),
\end{align}
where $\eta$ denotes the stepsize  and $R_{t,\mu} = \sum_{u=t}^T r_\mu(S_u,A_u)$.
%
Likewise, for problem \eqref{eqn_agmt_obj}, the stochastic approximation of gradient ascent yields
\begin{align}\label{update_rule_path}
    \theta_{k+1} = \theta_k + \eta \left( \hat{\nabla}_\theta V(\theta_k) +  \lambda \hat{\nabla}_\theta \mathbb{P} \left(\bigcap\limits_{t=0}^{T} \{ S_t \in \mathcal{S}_\text{safe}\}\right)   \right),
\end{align}
%
where the first term in bracket on the right-hand side is computed using \eqref{eqn_classical_PG_estimator} and the second term takes the form in  \eqref{eqn_theorem_estimator}.
%%








% \red{
% For this scenario, we take into account both formulations, namely, solving problems \eqref{eqn_problem1} and \eqref{eqn_problem2_mirror}. Recall that the only difference in two settings are the safety constraints and their relationship has been formally discussed in Section~\ref{Losses_of_Imposing_Relaxation}. We aim to use this simple example to numerically illustrate and compare the solutions of the two formulations. 

% It is important to point out that, the comparison is in terms of formulations but not algorithms. Indeed, as explained in Section~\ref{Losses_of_Imposing_Relaxation}, other algorithms in the literature attempt altogether to solve problem~\eqref{eqn_problem2_mirror}, different from problem~\eqref{eqn_problem1} that is of our interest.}

% \red{
% To solve the RL problem with cumulative safety constraints, i.e., problem~\eqref{eqn_problem2_mirror} iteratively, one can consider a reward shaping as follows
% \begin{equation}\label{eqn_reward_risk}
%   r_\mu(S_t, A_t)=r(S_t, A_t) + \mu r_c(S_t,A_t),
% \end{equation}
%  Based on $\mu$ one can maximize a novel cumulative reward 
% %
% \begin{equation}
%     V_\mu(\theta) = \mathbb{E} \left[\sum\limits_{t=0}^{T} \Big(r(S_t,A_t) + \mu r_c( S_t,A_t) \Big) |\pi_\theta \right].
% \end{equation}
% %
% There exist several algorithms~\cite{borkar2005actor,bhatnagar2012online,liang2018accelerated,tessler2018reward} that combine RL algorithms to perform the maximization of $V_\mu(\theta)$ with optimization algorithms to update the coefficient $\mu$. On the other hand, employing Policy Gradient Theorem and stochastic approximation provides us the following update rule for the parameters $\theta$ of the policy
% \begin{align}\label{update_rule_cumulative}
%     \theta_{k+1} &=\theta_k + \eta  \hat{\nabla} V_\mu (\theta) \nonumber \\
%     &= \theta_k+\eta\left(\sum\limits_{t=0}^{T-1} R_{t,\mu} \nabla_{\theta}\log\pi_\theta(A_t\mid S_t) \right),
% \end{align}
% where $\eta$ denotes the stepsize  and $R_{t,\mu} = \sum_{u=t}^T r(S_u,A_u) + \mu \mathbbm{1}(S_u\in \mathcal{S}_{\text{safe}}$).  
% Likewise, we combine \eqref{eqn_classical_PG_estimator} with \eqref{eqn_theorem_estimator} weighted by $\mu$ to construct the update rule for solving problem~\eqref{eqn_problem1}
% \begin{align}\label{update_rule_path}
%     \theta_{k+1} = \theta_k + \eta \left( \hat{\nabla}_\theta V(\theta_k) +  \mu \hat{\nabla}_\theta \mathbb{P} \left(\bigcap\limits_{t=0}^{T} \{ S_t \in \mathcal{S}_\text{safe}\}\right)   \right).
% \end{align}
% }








Figure~\ref{configuration} demonstrates that the agent with probabilistic safety constraints is trained to safely navigate to the goal position (9, 1.5) from the initial state (1, 8.5) after 40,000 episodes of training, during which $\lambda$ is fixed to be 6 and with $\eta = 0.002$.

As mentioned in Section~\ref{Losses_of_Imposing_Relaxation}, $\mu$ and $\lambda$ trade-off performance in task completion and safety. It is important to point out that to attain the same level of safety, in general, different values of $\lambda$ and $\mu$ are required. We run algorithms \eqref{update_rule_cumulative} and \eqref{update_rule_path} with different weights $\mu,\lambda \in (0, 14]$ to find solutions to problems \eqref{eqn_relaxation_2} and \eqref{eqn_agmt_obj} respectively. For different values of $\lambda$ and $\mu$ different optimal step-sizes can be used which results in faster or slower convergence of the algorithms. The worst case scenario requires $\eta = 0.0006$. In this case 2,000,000 episodes are needed.

%
The level of safety is the fraction of safe episodes (with all their states in the safe set as per Definition \ref{definition_safety}) that the trained policy yields over 1000 independent episodes under different random seeds. The initial state is uniformly drawn from the safe set for each episode. Similarly, we evaluate the value function by averaging the cumulative reward across the evaluation episodes.

The scatter plot in Figure~\ref{safety_vs_reward} depicts the results of the safety and average reward for problems \eqref{eqn_agmt_obj} and \eqref{eqn_relaxation_2} for different values $\lambda, \mu \in [0.45, 14]$. Observe that in both formulations, the higher the desired safety, the lower the average reward is. Despite this common trend, for the same level of safety, the probabilistic constrained problem yields an overall larger average reward. Hence, demonstrating empirically, that the probabilistic constraint formulation yields a better safety-performance trade-off. This result is in accordance with the theoretical bounds provided in Theorem~\ref{corollary_P_star_Ptilder_star}. It is worth pointing that the curve of reward-safety in Figure~\ref{safety_vs_reward} is approximately concave, and shows an empirical evidence of the concavity of $\tilde{P}^\star(\xi)$ in \eqref{eqn_problem2} with respect to $\xi$.

Notice that the algorithms used in this numerical section are Monte Carlo methods~\cite[Chapter 5]{sutton2018reinforcement}. In the RL literature there exist algorithms that exploit temporal differences~\cite{watkins1992q} and/or trust regions~\cite{schulman2015trust} which result in faster convergence rates. The goal of this numerical section is not to show faster convergence but to demonstrate the theoretical underpinnings established in Section III as well as to show that the estimation of the gradient of the probabilistic constraints (Theorem~\ref{theorem_safe_policy_gradient}) can successfully be employed for solving the task at hand. As mentioned in Section \ref{Gradient of the Probabilistic Constraint} the estimation of the gradient of the probabilistic constraint is zero for every unsafe episode. Thus hindering the rate of convergence. Analyzing alternatives to overcome this issue is out of the scope of this work.

